Multi-stream Fusion for Class Incremental Learning in Pill Image Classification

Classifying pill categories from real-world images is crucial for various smart healthcare applications. Although existing approaches in image classification might achieve a good performance on fixed pill categories, they fail to handle novel instances of pill categories that are frequently presented to the learning algorithm. To this end, a trivial solution is to train the model with novel classes. However, this may result in a phenomenon known as catastrophic forgetting, in which the system forgets what it learned in previous classes. In this paper, we address this challenge by introducing the class incremental learning (CIL) ability to traditional pill image classification systems. Specifically, we propose a novel incremental multi-stream intermediate fusion framework enabling incorporation of an additional guidance information stream that best matches the domain of the problem into various state-of-the-art CIL methods. From this framework, we consider color-specific information of pill images as a guidance stream and devise an approach, namely "Color Guidance with Multi-stream intermediate fusion"(CG-IMIF) for solving CIL pill image classification task. We conduct comprehensive experiments on real-world incremental pill image classification dataset, namely VAIPE-PCIL, and find that the CG-IMIF consistently outperforms several state-of-the-art methods by a large margin in different task settings. Our code, data, and trained model are available at https://github.com/vinuni-vishc/CG-IMIF.

==> methodology.tex <==
The majority of current pill identification methods relies on RGB images. Therefore, to the best of our knowledge, most existing systems fail to address hard examples (\textit{e.g}, pills with very similar shapes and colors)~\cite{9157392}. This problem becomes more challenging in the context of the class incremental learning. In this problem, we have to cope with two issues at the same time: 1) recognizing pill instances that belong to the novel classes, and 2) not forgetting the previously learned knowledge of the old ones.
We seek in this study robust domain-specific knowledge, which could be in good companion with traditional RGB image stream. However, the introduction of an additional stream issue a different challenge; the significant need for a stream integration method . To tackle such a challenge, we propose an Incremental Multi-stream Intermediate Fusion framework (IMIF). The IMIF allows additional information streams to be effectively propagated during the incremental learning phase. In the following subsections, we briefly define the multi-stream class incremental learning method and describe how it can be decomposed into different components.

\subsection{Multi-stream Class Incremental Learning Model}

We define a multi-stream class incremental learning model \textbf{M} as a combination of three key components: 1) a single stream base method \textbf{X}, 2) an additional stream of information \textbf{Y}, and 3) a method of fusing stream \textbf{Z}.


\begin{center}
    \textbf{M} = Base method \textbf{X} + Feature stream \textbf{Y} + Fusion mechanism \textbf{Z}
\end{center}

At this point, the base method represents any method that follows the general setting described in Sec.\ref{subsec:conventionalCIL}. \textbf{Y} serves as a piece of additional domain information that gives cues to the learning model apart from RGB images. 
Normally, \textbf{Y} is specific to the domain of the task. Lastly, \textbf{Z} presents a fusion mechanism that enables method \textbf{M} to incorporate additional information stream \textbf{Y} into the incremental learning process. From this decomposition, our CG-IMIF replaces: 1) the representative stream \textbf{Y} with color-specific information, and 2) the fusion technique \textbf{Z} with the proposed IMIF.
In the following, we describe our proposed Color histogram guidance stream and Incremental Multi-stream Intermediate Fusion technique in Sec.\ref{ssec:domain-specific information extractor} and Sec.\ref{subsec:fusion}, respectively.

% \subsection{Base Method X}

% At this point, base method X can be represented with any exemplar-based methods which follows the general architecture described in Sec.\ref{subsec:conventionalCIL}.

% Baseline methods are those existing works that have been proposed to solve the traditional \textcolor{blue}{\st{Class Incremental Learning}} \textcolor{red}{CIL} problem. \textcolor{red}{In the task of the prescription pill images}, we inherited various exemplar-based class incremental learning approaches to study the effect of \textcolor{blue}{\st{our}} \textcolor{red}{[Please do not use too much "our"]} the proposed framework IMIF when being integrated into the original one. In general, most of the exemplar-based CIL methods \textcolor{blue}{\st{would follow to}} consist of two following components:


\subsection{Color Histogram Guidance Stream} \label{ssec:domain-specific information extractor}

Pill images compose of various features which can be used as discriminative factors in classification problems. Among those is color distribution information which can be approximated by the color histogram of pill images. The color histogram represents the color distribution of the input image in terms of three different channels: red, green, and blue. In detail, it is often encoded into a single vector where the indexes of entries are mapped to a set of all possible colors. In grey-scale images, values of vector entries store the frequency that counts the total number of pixels having the intensity (\textit{i.e.}, color value), which is hashed by the corresponding index of the vector. However, in a three-dimensional image, color ranges for each channel are associated across color channels to formulate a unique combination. This combination accounts for those pixels of which color ranges lie in three discrete ranges of value: $[r_i, r_j];[g_k, g_l];[b_m, b_n]$. The color feature vectors are useful to make a distinction among pill instances that have similar shapes but different colors. The color ranges for each channel of the RGB images are divided into eight segments in our problem, where each segment represents 32 different consecutive color values. After that, the color histogram vector can be obtained by accumulating the quantities of pixels assigned to a specific color range for each channel to result in a vector with 8$\times$8$\times$8 = 512 elements. Fig.~\ref{fig:example_color_histogram} illustrates a few examples of extracting the color histogram stream for each corresponding cropped pill image.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.5\textwidth]{images/ColorHistogram.pdf}
    \caption{Samples of pill images from VAIPE-PCIL dataset are shown on the first row. Second row exhibits the corresponding color histogram information for images on the upper row respectively.}
    \label{fig:example_color_histogram}
\end{figure}

\subsection{Incremental Multi-stream Intermediate Fusion Technique}
\label{subsec:fusion}

\subsubsection{Traditional Early Fusion}
A naive fusion technique \textbf{Z} concatenates different streams of information right after the feature extraction phase. Specifically, feature vectors $f_{r} \in \mathbb{R}^{d_r}$, and $f_Y \in \mathbb{R}^{d_Y}$ are extracted from raw RGB images, and additional information stream \textbf{Y}, respectively. Both of these features are then fed into separate projection layers to project into the same latent space. In practice, the projection layers are implemented by a single hidden layer controlled by parameters $\Theta^p=[W^p, b^p]$ as follows
\begin{equation}
s_{r} = \sigma(W^p_r.f_r+b^p_r),\\  s_{Y} =\sigma(W^p_Y.f_Y+b^p_Y), \\  s_{g} = [s_r, s_Y].
\label{eq:projection_layer}
\end{equation}
The projected vectors are then concatenated to obtain the global feature vector $s_g \in \mathbb{R}^{d_g}$. This global feature $s_g$ can be considered as a single input into any traditional single stream CIL methods as shown in Fig.~\ref{fig:traditional_single_stream}.
\begin{figure}[h!]
    \centering
    \includegraphics[width=10cm,height=5cm]{images/traditional_single_stream.pdf}
    \caption{The traditional training paradigm with only single-stream information use by almost existing exemplar-based CIL methods.}
    \label{fig:traditional_single_stream}
\end{figure}
\noindent \subsubsection{Intermediate Fusion}
We observed and hypothesized that fusing information stream in an early manner for a class incremental learning problem is not optimal. The global feature $s_g$ is problematic since it is regularly updated at each incremental task. As a result, the projection layer in the early phase can not find good parameters that balance the performance of old and novel categories in different tasks. Therefore, we propose to relocate the projection layer to the intermediate phase instead (\textit{i.e}, incremental learning phase) by initiating an entirely novel projection layer in an incremental manner. When $C^t$ from new task $t$ arrives at the system, a new classification layer $CL_t$ is created . This layer accompanies with an attached projection layer specific to the information stream of a specific task. Therefore, the parameters controlling the projection layer for each information stream are different from those defined in the early fusion.

\begin{equation} 
\Theta^{p^t}_{r} = [W^{p^t}_r, b^{p^t}_r],
\Theta^{p^t}_{Y} = [W^{p^t}_Y, b^{p^t}_Y].
\end{equation}

In this way, the projection layer could maintain its optimal performance for old tasks without significantly adjusting its weight toward the novel ones. Fig.~\ref{fig:our_X_CG_IMIF} illustrates how we direct streams of additional knowledge in an incremental manner.
\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{images/X-CG-IMIF.pdf}
    \caption{Our proposed CG-IMIF architecture composes of: 1) color histogram feature extraction (orange block), and 2) intermediate fusion framework (purple block) to incorporate additional information stream.}
    \label{fig:our_X_CG_IMIF}
\end{figure}
